EBV-CAN: Vision--Language Grounding for Contact-Aided Endoscope Navigation

Flexible endoscopes exploit structural compliance to traverse narrow lumens, pipes, and cavities, where navigation involves distributed environmental contact. This compliance makes tip motion depend on the evolving support configuration. We present external bird's-eye-view contact-aided navigation (EBV-CAN), a vision-language policy that combines one initial global static bird's-eye image with evolving endoscopic observations and motor state. Three supervised semantic queries locate the tip, next waypoint, and instructed target on the cached global image; their residual representations predict bending and insertion commands. We introduce the Vision-Language Contact-Aided (VLCA) dataset, linking 517 demonstrations and 75k action samples to 958k spatial entries and 93k remaining-route records. On 50 held-out episodes, tip-coordinate and waypoint localization reach 97.5% and 94.8%. Swapping the target instruction under identical observations changes target attention and motor output across 17 dual-target episodes. Across 1,920 physical trials of eight policies trained under a shared protocol, EBV-CAN achieves 183/240 successes (76.25%) under automatic blue-area scoring. Gated recurrent unit behavior cloning (GRU-BC) achieves the lowest matched-task offline mean absolute error (MAE), 0.056, and 1/240 physical successes, establishing distinct rankings for action imitation and task completion. Successful multi-guide executions and representative failures connect spatial progress, steering transitions, and visibility to physical navigation.

==> vendor/bibunits/README <==
Abstract

  The `bibunits' package allows separate bibliographies for different
  units or parts of the text. The units can be chapters, sections or
  bibunit environments. The package is compatible with a wide variety of
  packages, including, but not limited to, natbib, overcite and
  KOMA-SCRIPT classes.


To produce the style
  
  latex bibunits.ins


To produce the documentation

  latex bibunits.dtx

  If you do not want to include the macro section in the documentation,
  remove the comment sign before \OnlyDescription.


  To produce an index for the documentation:

    makeindex -s gind.ist bibunits

  To produce a change history for the documentation:
  
    makeindex -s gglo.ist -o bibunits.gls bibunits.glo


Contents:
 
  00Readme      this file ;-)
  bibunits.dtx  documented source file for the bibunits package
  bibunits.ins  installation file
  bibtexall     shell script to run bibtex on each .aux file in the
                   present directory


License

  Package `bibunits' to use with LaTeX2e.

  Copyright (C) 1999--2004 Thorsten Hansen

  This work may be distributed and/or modified under the conditions of
  the LaTeX Project Public License, either version 1.3 of this license
  or any later version. The latest version of this license is in
  http://www.latex-project.org/lppl.txt and version 1.3 or later is
  part of all distributions of LaTeX version 2003/12/01 or
  later.
  
  This work has the LPPL maintenance status "maintained". The Current
  Maintainer of this work is Thorsten Hansen.
  
  This work consists of the files bibunits.dtx and bibunits.ins
  and the derived file bibunits.sty.




Happy TeXing

    Thorsten Hansen
    thorsten.hansen@psychol.uni-giessen.de

